AGNIFS survey of local AGN: GMOS-IFU data and outflows in 30 sources

We analyse optical datacubes of the inner kiloparsec of 30 local ($z\le0.02$) active galactic nuclei (AGN) hosts that our research group, AGNIFS, has collected over the past decade via observations with the integral field units of the Gemini Multi-Object Spectrographs. Spatial resolutions range between $50~{\rm pc}$ and $300~{\rm pc}$ and spectral coverage is from $4800~\mathring{A}$ or $5600~\mathring{A}$ to $7000~\mathring{A}$, at velocity resolutions of $\approx 50~{\rm km~s^{-1}}$. We derive maps of the gas excitation and kinematics, determine the AGN ionisation axis -- which has random orientation relative to the galaxy, and the kinematic major axes of the emitting gas. We find that rotation dominates the gas kinematics in most cases, but is disturbed by the presence of inflows and outflows. Outflows have been found in 21 nuclei, usually along the ionisation axis. The gas velocity dispersion is traced by $W_{80}$ (velocity width encompassing 80 per cent of the line flux), adopted as a tracer of outflows. In 7 sources $W_{80}$ is enhanced perpendicularly to the ionisation axis, indicating lateral expansion of the outflow. We have estimated mass-outflow rates $\dot{M}$ and powers $\dot{E}$, finding median values of $\log\,[\dot{M}/({\rm\,M_\odot\,yr^{-1}})]=-2.1_{-1.0}^{+1.6}$ and $\log\,[\dot{E}/({\rm\,erg\,s^{-1}})]=38.5_{-0.9}^{+1.8}$, respectively. Both quantities show a mild correlation with the AGN luminosity ($L_{\rm AGN}$). $\dot{E}$ is of the order of 0.01 $L_{\rm AGN}$ for 4 sources, but much lower for the majority (9) of the sources, with a median value of $\log\,[\dot{E}/L_{\rm AGN}]=-5.34_{-0.9}^{+3.2}$ indicating that typical outflows in the local Universe are unlikely to significantly impact their host galaxy evolution.

==> ser_sizes.tex <==
\begin{table}
\caption{Strong emission region sizes}
\label{tab:ser_sizes}
\begin{tabular}{lcc}
\hline
\hline
Galaxy & $R_{\rm max}$ [N II] & $R_{\rm max}$ [O III] \\
 & pc & pc \\
\hline
Mrk~348 & 85 & 96 \\
NGC~1068 & 152 & 139 \\
Mrk~1058 & 612 & 528 \\
Mrk~607 & 224 & 252 \\
NGC~1365 & 258 & 289 \\
NGC~1358 & 748 & -- \\
NGC~1386 & 263 & -- \\
NGC~1566 & 19 & -- \\
NGC~1667 & 285 & -- \\
NGC~2110 & 479 & -- \\
Mrk~6 & 584 & 561 \\
Mrk~79 & 1199 & 1123 \\
NGC~2787 & 38 & -- \\
MCG~-05-23-016 & 245 & 281 \\
NGC~3081 & 273 & -- \\
NGC~3227 & 82 & 85 \\
NGC~3516 & 934 & 264 \\
NGC~3783 & 257 & 303 \\
NGC~3786 & 251 & 251 \\
NGC~3982 & 106 & -- \\
NGC~4180 & 406 & -- \\
NGC~4450 & 90 & -- \\
NGC~4501 & 183 & -- \\
NGC~4593 & 127 & 112 \\
MCG~-06-30-015 & 177 & 36 \\
NGC~5728 & 358 & 334 \\
NGC~5899 & 275 & 290 \\
NGC~6300 & 112 & 139 \\
NGC~6814 & 149 & 153 \\
NGC~7213 & 57 & -- \\
\hline
\end{tabular}
\end{table}

